Disco: A Functional Programming Language for Discrete Mathematics

Disco is a pure, strict, statically typed functional programming language designed to be used in the setting of a discrete mathematics course. The goals of the language are to introduce students to functional programming concepts early, and to enhance their learning of mathematics by providing a computational platform for them to play with. It features mathematically-inspired notation, property-based testing, equirecursive algebraic types, subtyping, built-in list, bag, and finite set types, a REPL, and student-focused documentation. Disco is implemented in Haskell, with source code available on GitHub [https://github.com/disco-lang/disco], and interactive web-based REPL available through replit [https://replit.com/@BrentYorgey/Disco#README.md].

==> eptcsdata.tex <==
\providecommand{\firstpage}{64}
\providecommand{\publicationstatus}{Elena Machkasova (Ed.): International Workshop on Trends\\
in Functional Programming in Education 2023 (TFPIE 2023)\\
EPTCS 382, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.382.4}{10.4204/EPTCS.382.4}}

